Defending Against Adversarial Attacks in Transmission- and Distribution-level PMU Data

Phasor measurement units (PMUs) provide high-fidelity data that improve situation awareness of electric power grid operations. PMU datastreams inform wide-area state estimation, monitor area control error, and facilitate event detection in real time. As PMU data become more available and increasingly reliable, these devices are found in new roles within control systems, such as remedial action schemes and early warning detection systems. As with other cyber physical systems, maintaining data integrity and security pose a significant challenge for power system operators. In this paper, we present a comprehensive analysis of multiple machine learning techniques to detect malicious data injection within PMU data streams. The two datasets used in this study come from two PMU networks: an inter-university, research-grade distribution network spanning three institutions in the U.S. Pacific Northwest, and a utility transmission network from the Bonneville Power Administration. We implement the detection algorithms with TensorFlow, an open-source software library for machine learning, and the results demonstrate potential for distributing the training workload and achieving higher performance, while maintaining effectiveness in the detection of spoofed data.

==> 0_preface.tex <==
\section{Preface -- This should be pulled out into a cover letter eventually}

\subsection{Comments from the Reviews}


{\em TSUSC-2018-10-0114, ``Defending Against Adversarial Attacks in Transmission- and Distribution-level PMU Data''}

09-May-2019

Dear Dr. Zhao,

We now have reviews of your above referenced submission to IEEE Transactions on Sustainable Computing. Copies of the review comments are enclosed.

After considering the reviews and recommendation of the Associate Editor, I have determined that you should revise the paper as per review comments and resubmit as a new paper. The history of the paper will be preserved, but, it will be treated as a NEW submission and given a new log number.

If you choose to revise and resubmit your paper, please include this original log number TSUSC-2018-10-0114 when submitting and include a detailed summary of the changes you made in response to the AE and reviewers comments. We will include your previous manuscript's history in its files. The AE may choose to send the paper to the original reviewers so that the continuity is preserved.

The Associate Editor has the following comments for you:

{\em Associate Editor
Comments to the Author:
There are three reviewers expressing diverse opinions about the paper. However, it is noteworthily mentioning that the two expert reviewers gave rather negative reviews. They questioned the clarity and correctness of this work. Also, one reviewer concerns the differences between transmission PMU and distribution PMU. Furthermore, this paper appears to be short of results, as compared with other papers that are invited to this special issue from ACM eEnergy (which is a very competitive conference). The authors are encouraged to strengthen their work and consider to submit to this journal as a new submission in future.}

We hope that you will find the comments from the reviewers to be useful in your future work.  If you have any questions, feel free to contact us.

Sincerely,

Albert Zomaya, EIC
Transactions on Sustainable Computing
albert.zomaya@sydney.edu.au


\subsection{Reviewers' Comments}

Please note that some reviewers may have included additional comments in a separate file. If a review contains the note ``see the attached file'' under Section III A - Public Comments, you will need to log on to ScholarOne Manuscripts  to view the file. After logging in, select the Author Center, click on the "Manuscripts with Decisions" queue and then clicking on the "view decision letter" link for this manuscript. You must scroll down to the very bottom of the letter to see the file(s), if any.  This will open the file that the reviewer(s) or the Associate Editor included for you along with their review.

\subsection{Reviewer: 1}

Recommendation: {\em Author Should Prepare A Minor Revision}

{\em Comments:}
I enjoyed reading this paper. It provided a good introduction to phasor measurement units and it explained the problem well. It makes sense to me that utilities might want to implement this method or something similar on their electrical networks.

In section IV.C. you say it takes 8 CPU cores to compute correlations in real time. This seems like an excessive amount of work. The power distribution company will have to buy and maintain a \$2000-3000 computer for every subsection of the distribution network. If we increase the size of the subnetwork that we're studying above 10 PMUs, the computational complexity of computing these correlations gets worse fast. It may make the technique impractical, and I think you should address how to solve this problem. At a minimum, talk about how much effort this will take and if the cost of maintaining these machines will be worth the benefit of detecting spoofs.

\color{orange}

Our previous study shows that for the spoof detection purposes, it is not necessary to calculate correlations for all PMU pairs, because a small number of PMUs that are electrically close to the spoofed PMU will be enough for the algorithm to trigger the detection. In addition, these experiments are based on continuously calculating correlations using a 300-cycle sliding window with a step of 1 cycle. In reality, the sliding window can be adjusted by using larger steps, representing a trade off between the granularity of the correlations and the computational performance. Therefore, scalability is not an issue here. These explanations have been included in the revised version. 

\color{black}

Top of page 6, left column: excellent explanation of the hurdles that an attacker would need to overcome to spoof your detection scheme. I am curious if this is a tractable problem. This work assumes that the attacker has access to high-resolution data from a single PMU to create the spoof, which already seems like a high barrier to overcome (how would one get that?). If the attacker is sophisticated enough to get high-res data from a single PMU, can we assume that they can get time-synchronized data from multiple PMUs too?

\color{orange}

We do not make an assumption that the attacker has access to high-resolution data from a single PMU. We designed our spoof strategy, e.g., mirror, time dilation etc., using real PMU data to demonstrate the effectiveness of our detection algorithm. A spoof that is created using real high-resolution PMU data is harder to detect. If the attacker does not have the real PMU data, it is easier for the algorithm to detect the spoof. In the extremely rare case where attackers have access to multiple PMUs, we argue that it is difficult for them to spoof all PMUs while maintaining the original pair-wise correlations for all PMU pairs. Our algorithm is based on monitoring these correlations over time, and once there is a change in these correlations, the algorithm will detect this change. This has been explained in the revised version. 

\color{black}

Grammatical/Formatting notes:

\begin{itemize}
\item Page 2, Line 14, right column: A cyber attack on these PMU would...: should say "PMUs"

\color{orange}
Fixed. 
\color{black}

\item Page 2, Line 31, right column: it models spoof detection using dc power flow state estimators: DC should be capitalized. There are many more of these. Check for lower case ac also.
\item Page 4, Line 49, right column: 10 pmus each with 5 signals: should say PMUs

\color{orange}
Fixed. 
\color{black}

\item Page 5, Line 2, left column: an SVMs is supervised learning model with... should read "An SVM is a supervised learning model"

\color{orange}
Fixed. 
\color{black}

\end{itemize}


Additional Questions:

\begin{itemize}
    \item Which category describes this manuscript?: Research

\item 1. How relevant is this manuscript to the readers? Explain under Public Comments: Relevant

\item 1. Please explain how this manuscript advances this field of research and/or contributes something new to the literature.: In this work, the authors discuss a new method for detecting false data injection in networks of phasor measurement units. The authors argue that PMUs are susceptible to single-point data injection attacks which could compromise the stability of an electrical transmission or distribution network. The authors present three possible modes of attack: mirroring, repeated last value, and time dilation. They demonstrate how to detect these attack modes by comparing PMU readings in a local network. It appears that the technique of using large datasets coupled with machine learning is new in this body of work.

\item 2. Is the manuscript technically sound? Please explain your answer under Public Comments below.: Yes

\item 1. Are the title, abstract, and keywords appropriate? Please explain under Public Comments below.: Yes

\item 2. Does the manuscript contain sufficient and appropriate references? Please explain under Public Comments below.: References are sufficient and appropriate

\item 3. Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? Please explain your answer under Public Comments below.: Yes

\item 4. How would you rate the organization of the manuscript? Is it focused? Is the length appropriate for the topic? Please explain under Public Comments below.: Could be improved

\item  5. Please rate the readability of the manuscript. Explain your rating under Public Comments below.: Easy to read

\item 6. Should the supplemental material be included? (Click on the Supplementary Files icon to view files): No, it should not be included at all

\item 7. If yes to 6 (above), should it be accepted: After revisions.  Please include explanation under Public Comments below.
\end{itemize}

Please rate the manuscript. Explain your choice.: {\bf Good}


\subsection{Reviewer: 2}

Recommendation: {\em Author Should Prepare A Major Revision For A Second Review}

{\em Comments:}
In order to detect spoofing in PMU data, this paper uses machine learning techniques to inspect the correlation of data from nearby PMUs. Three possible spoofing strategies, Repeated-Last-Value, Mirroring, and Time-Dilation, are considered. Simulations are used to show the performance of the proposed detecting methods.

This paper does show a novel method to detect PMU data spoofing, while some key parts lack clear enough explanation. Here are the detailed concerns.

\begin{itemize}
\item The proposed method in this paper needs data from multiple PMU. Does other work also need data from multiple PMU? I have this concern because, if multiple PMU data are needed, then the detection algorithm can only run at the control center, i.e., in a centralized way. In contrast, if only local PMU data are needed, then the detection algorithm can run in a distributed way, which is more preferable.

\blue{We've further clarified that our system runs using data from multiple PMUs in the introduction and added text in the related work section to indicate that most other spoof detection systems share this requirement. } 

\item The second constraint in the first paragraph of Section IV.A is unclear. Does this constraint imply the monotonicity of $s(t)$ with respect to t? If so, then why the true signal must be monotone?

\blue{No, the second constraint indicates that: {\em ``the onset of a spoof should not create a discontinuity--that is, a signal $s$ sampled immediately before the spoof, $s(t-1) = s_{true}(t-1)$, and at the start of the spoof $s(t) = s_{spoof}(t)$, should show a change in value that is consistent with historical movement of that signal.''} This does not imply monotonicity of $s(t)$ with respect to $t$ either before or after the spoof. It simply requires that the step in two adjacent measurements should not itself give away the spoof.  That is, for any $k>=t$, $|s(k)-s({k-1})|$ should be selected from the range of values observable when $k<t$. Note also that we've changed the notation for the time series from $s_t$ to $s(t)$ with the aim of clarifying the points below.} 

\item In the fourth paragraph of section IV.A, please define the first derivative of $s(t)$ (note that t is discrete here). Do you mean something like $s(t)'=s(t)-s(t-1)$?

\blue{Correct.  We've updated the notation to make that clear.}

\item Please explain why only these three spoofing strategies (Repeated-Last-Value, Mirroring, and Time-Dilation) is considered. Do those strategies appear in other literature? Do they have advantages over other possible strategies?

\blue{These spoofing strategies do appear in other literature, we've clarified that in text. Their advantages are listed in Paragraph 1 of Part A in the Methodology section (IV.A)}

\item  The time-dilation spoof stated in the last paragraph of Section IV.A is quite unclear. Please define the concepts such as "cycles" and "play back" used in this paragraph. An example of this spoof is highly recommended for better illustration.

\blue{We've added additional description in Section IV.A as well as a graphical illustration of the time-dilation spoof.}
\end{itemize}

Additional Questions:
\begin{itemize}
    \item Which category describes this manuscript?: Technology

\end{itemize}

How relevant is this manuscript to the readers? Explain under Public Comments: Relevant
\begin{itemize}
\item 1. Please explain how this manuscript advances this field of research and/or contributes something new to the literature.: 1. Use correlation to detect spoofing.

\item 1. Apply machine learning to real PMU data streams.

\item 2. Is the manuscript technically sound? Please explain your answer under Public Comments below.: Partially

\item 1. Are the title, abstract, and keywords appropriate? Please explain under Public Comments below.: Yes

\item 2. Does the manuscript contain sufficient and appropriate references? Please explain under Public Comments below.: References are sufficient and appropriate

\item 3. Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? Please explain your answer under Public Comments below.: Yes

\item 4. How would you rate the organization of the manuscript? Is it focused? Is the length appropriate for the topic? Please explain under Public Comments below.: Satisfactory

\item 5. Please rate the readability of the manuscript. Explain your rating under Public Comments below.: Readable - but requires some effort to understand

\item 6. Should the supplemental material be included? (Click on the Supplementary Files icon to view files): Does not apply, no supplementary files included

\item 7. If yes to 6 (above), should it be accepted:
\end{itemize}

Please rate the manuscript. Explain your choice.: Good


\subsection{Reviewer: 3}

Recommendation: Revise and Resubmit as “New”

Comments:
\begin{itemize}
\item Page 1 - Space missing column 2 "The second dataset"
\item Page 2 - Space missing column 1 "Second, to the best..."
\item Page 2 - Spelling "withing"
\item Page 2 - Gramma "As noted previously, PMU data have..."
\item Section F. Common Limitations - what is H?
\end{itemize}
{\em Major concerns -}
\begin{enumerate}

\color{orange}
\item No mention of Ukraine and associated literature on the topic.

\color{blue}
We've added mention of the 2015 Ukraine attack, and a reference, to Section II: 
\\ \\
``Another example of using false data to facilitate a cyber attack was the multifaceted 2015 disruption of generation facilities in Ukraine~\cite{7752958}. Operators were prevented from sending commands to remote SCADA devices because the attackers had corrupted those devices with malicious firmware. This prevented operators from bringing generation resources back online after the initial attack.''

\color{orange}
\item No mention of the \$77 million DARPA program on topic and the supporting literature - looking at impedance estimation to identify an attack.

\color{blue}
ECS: I assume they are talking about RADICS projects here? I haven't seen much literature to come out of it yet, but here are some ideas to trace: 

Pal, Seemita, Biplab Sikdar, and Joe H. Chow. ``Classification and detection of PMU data manipulation attacks using transmission line parameters.'' IEEE Transactions on Smart Grid 9, no. 5 (2017): 5057-5066.
(This above is also the group working on distribution level PMUs so we could use the reference for both comments) 

Davis, Katherine R., Charles M. Davis, Saman A. Zonouz, Rakesh B. Bobba, Robin Berthier, Luis Garcia, and Peter W. Sauer. ''A cyber-physical modeling and assessment framework for power grid infrastructures.'' IEEE Transactions on smart grid 6, no. 5 (2015): 2464-2475.

This group was also looking at probing in terms of line impedance, but they started with this: 
Estimation of transmission line parameters from historical data
KR Davis, S Dutta, TJ Overbye, J Gronquist
2013 46th Hawaii International Conference on System Sciences, 2151-2160

\color{orange}
\item No mention of False Data Injection Attacks and the supporting literature on the topic.
In general, the literature referenced is focused on pre-2015 before the Ukraine cyber incident, after which considerable literature on the topic followed.
\\
\color{blue}

ECS: Adding some references here to discuss. Added to smartgrid2.bib as well,

brahma2016real
S. Brahma, R. Kavasseri, H. Cao, N. R. Chaudhuri, T. Alexopoulos, andY.  Cui,  “Real-time  identification  of  dynamic  events  in  power  systems using  pmu  data,  and  potential  applications—models,  promises,  and challenges,” IEEE  transactions  on  Power  Delivery,  vol.  32,  no.  1,  pp.294–301, 2016

Yasinzadeh2018detection
M.  Yasinzadeh  and  M.  Akhbari,  “Detection  of  pmu  spoofing  in  powergrid based on phasor measurement analysis,” IET Generation, Transmis-sion Distribution, vol. 12, no. 9, pp. 1980–1987, 2018.


\color{orange}
\item No mention is made on the accuracy of distribution-level PMUs and what level of accuracy is needed to measure distribution phase angles.

\color{blue}
We have found that the quality of the phase angle resolution is the same for distribution and transmission level PMU data, and both are sufficient for calculating the Pearson Correlation between PMU data streams. We have not had issues calculating phase angles from distribution-level PMUs, and as such, we don't discuss the issue within the manuscript.

\color{orange}
\item No mention of the relevance of the positive sequence for distribution circuits is made - especially given distribution grids are not often balanced and the circuits are not typically transposed.

\color{blue} The positive sequence exists in a three phase system regardless of system balance or transposition.  It is highly relevant, in both transmission and distribution, as it is the component that carries apparent power.  Consider too that at the point of measurement, the substation, distribution systems are relatively balanced.  Even along the lengths of feeders, the positive sequence component remains by far the largest of the sequence components, and is readily available for correlation with nearby PMUs. 
\\
Lack of transposition is just another source of imbalance, which, if significant, would be captured in the negative sequence component. However, distribution lines are usually too short to justify transposition.  We don't see this as an issue of concern.  The manuscript demonstrates that we are able to use correlation of positive sequence phase angle from distribution PMUs effectively.

\color{orange}
\item In Section Feature Extraction, a stronger justification for the correlation approach is needed

In section V.B. paragraph 4, we discuss the degree of correlation of PMU data parameters between PMUs.  We note that ``correlation vectors $r(|V_+|)$, $r(\phi_+)$ and $r(f)$ are good candidates for detecting spoofing attacks, as these consistently exhibit moderate to high correlation values over wide ranges of time. The $r(\phi_+)$ correlation values are exceptionally high, near 1.0 under normal circumstances.''  We outline our methods and demonstrate results in more detail in another publication, a citation to which has been added at the end of this paragraph.

\color{orange}
\item Section E. Evaluation Metrics - no mention of data quality is made - signal drop out is common with PMU data - how might this impact the results?

\color{blue}
A paragraph was added discussing data drop and data drift issues, which are common with PMUs.  We now include a reference to a study that demonstrated that drop and drift are easily detected through the Pearson Correlation method described in this paper.
\\ \\
``PMU data can be unreliable, and this lack of reliability can affect the aforementioned metrics.  For instance, a PMU may go offline, resulting in so-called ``data drop,'' which appears as a stream of zero-value data.  Other times, a PMU may produce the same measurements over a continuous period, often termed ``data drift.''  When processing PMU data for analysis, data drop and drift periods need to be removed.  Correlation can help.  As demonstrated by Meier et al., both data drop and data drift are easily identified through rapid decorrelation between the faulting PMU and near-by PMUs [Meier].''

\end{enumerate}

Additional Questions:
1. Which category describes this manuscript?: Practice / Application / Case Study / Experience Report

How relevant is this manuscript to the readers? Explain under Public Comments: Interesting - but not very relevant

1. Please explain how this manuscript advances this field of research and/or contributes something new to the literature.: I don't feel the manuscript advances the field in this research area.

2. Is the manuscript technically sound? Please explain your answer under Public Comments below.: Partially

\begin{itemize}
    \item 1. Are the title, abstract, and keywords appropriate? Please explain under Public Comments below.: No

\item 2. Does the manuscript contain sufficient and appropriate references? Please explain under Public Comments below.: Important references are missing; more references are needed

\item 3. Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? Please explain your answer under Public Comments below.: Yes

\item 4. How would you rate the organization of the manuscript? Is it focused? Is the length appropriate for the topic? Please explain under Public Comments below.: Could be improved

\item 5. Please rate the readability of the manuscript. Explain your rating under Public Comments below.: Easy to read

\item 6. Should the supplemental material be included? (Click on the Supplementary Files icon to view files): No, it should not be included at all

\item 7. If yes to 6 (above), should it be accepted: After revisions.  Please include explanation under Public Comments below.
\end{itemize}

Please rate the manuscript. Explain your choice.: {\em Fair}



==> 6_discussion.tex <==
\section{Discussion}\label{sec:discussion}

==> PMU data/0_preface.tex <==
\section{Preface -- This should be pulled out into a cover letter eventually}

\subsection{Comments from the Reviews}


{\em TSUSC-2018-10-0114, ``Defending Against Adversarial Attacks in Transmission- and Distribution-level PMU Data''}

09-May-2019

Dear Dr. Zhao,

We now have reviews of your above referenced submission to IEEE Transactions on Sustainable Computing. Copies of the review comments are enclosed.

After considering the reviews and recommendation of the Associate Editor, I have determined that you should revise the paper as per review comments and resubmit as a new paper. The history of the paper will be preserved, but, it will be treated as a NEW submission and given a new log number.

If you choose to revise and resubmit your paper, please include this original log number TSUSC-2018-10-0114 when submitting and include a detailed summary of the changes you made in response to the AE and reviewers comments. We will include your previous manuscript's history in its files. The AE may choose to send the paper to the original reviewers so that the continuity is preserved.

The Associate Editor has the following comments for you:

{\em Associate Editor
Comments to the Author:
There are three reviewers expressing diverse opinions about the paper. However, it is noteworthily mentioning that the two expert reviewers gave rather negative reviews. They questioned the clarity and correctness of this work. Also, one reviewer concerns the differences between transmission PMU and distribution PMU. Furthermore, this paper appears to be short of results, as compared with other papers that are invited to this special issue from ACM eEnergy (which is a very competitive conference). The authors are encouraged to strengthen their work and consider to submit to this journal as a new submission in future.}

We hope that you will find the comments from the reviewers to be useful in your future work.  If you have any questions, feel free to contact us.

Sincerely,

Albert Zomaya, EIC
Transactions on Sustainable Computing
albert.zomaya@sydney.edu.au


\subsection{Reviewers' Comments}

Please note that some reviewers may have included additional comments in a separate file. If a review contains the note ``see the attached file'' under Section III A - Public Comments, you will need to log on to ScholarOne Manuscripts  to view the file. After logging in, select the Author Center, click on the "Manuscripts with Decisions" queue and then clicking on the "view decision letter" link for this manuscript. You must scroll down to the very bottom of the letter to see the file(s), if any.  This will open the file that the reviewer(s) or the Associate Editor included for you along with their review.

\subsection{Reviewer: 1}

Recommendation: {\em Author Should Prepare A Minor Revision}

{\em Comments:}
I enjoyed reading this paper. It provided a good introduction to phasor measurement units and it explained the problem well. It makes sense to me that utilities might want to implement this method or something similar on their electrical networks.

In section IV.C. you say it takes 8 CPU cores to compute correlations in real time. This seems like an excessive amount of work. The power distribution company will have to buy and maintain a \$2000-3000 computer for every subsection of the distribution network. If we increase the size of the subnetwork that we're studying above 10 PMUs, the computational complexity of computing these correlations gets worse fast. It may make the technique impractical, and I think you should address how to solve this problem. At a minimum, talk about how much effort this will take and if the cost of maintaining these machines will be worth the benefit of detecting spoofs.

\color{orange}

Our previous study shows that for the spoof detection purposes, it is not necessary to calculate correlations for all PMU pairs, because a small number of PMUs that are electrically close to the spoofed PMU will be enough for the algorithm to trigger the detection. In addition, these experiments are based on continuously calculating correlations using a 300-cycle sliding window with a step of 1 cycle. In reality, the sliding window can be adjusted by using larger steps, representing a trade off between the granularity of the correlations and the computational performance. Therefore, scalability is not an issue here. These explanations have been included in the revised version. 

\color{black}

Top of page 6, left column: excellent explanation of the hurdles that an attacker would need to overcome to spoof your detection scheme. I am curious if this is a tractable problem. This work assumes that the attacker has access to high-resolution data from a single PMU to create the spoof, which already seems like a high barrier to overcome (how would one get that?). If the attacker is sophisticated enough to get high-res data from a single PMU, can we assume that they can get time-synchronized data from multiple PMUs too?

\color{orange}

We do not make an assumption that the attacker has access to high-resolution data from a single PMU. We designed our spoof strategy, e.g., mirror, time dilation etc., using real PMU data to demonstrate the effectiveness of our detection algorithm. A spoof that is created using real high-resolution PMU data is harder to detect. If the attacker does not have the real PMU data, it is easier for the algorithm to detect the spoof. In the extremely rare case where attackers have access to multiple PMUs, we argue that it is difficult for them to spoof all PMUs while maintaining the original pair-wise correlations for all PMU pairs. Our algorithm is based on monitoring these correlations over time, and once there is a change in these correlations, the algorithm will detect this change. This has been explained in the revised version. 

\color{black}

Grammatical/Formatting notes:

\begin{itemize}
\item Page 2, Line 14, right column: A cyber attack on these PMU would...: should say "PMUs"

\color{orange}
Fixed. 
\color{black}

\item Page 2, Line 31, right column: it models spoof detection using dc power flow state estimators: DC should be capitalized. There are many more of these. Check for lower case ac also.
\item Page 4, Line 49, right column: 10 pmus each with 5 signals: should say PMUs

\color{orange}
Fixed. 
\color{black}

\item Page 5, Line 2, left column: an SVMs is supervised learning model with... should read "An SVM is a supervised learning model"

\color{orange}
Fixed. 
\color{black}

\end{itemize}


Additional Questions:

\begin{itemize}
    \item Which category describes this manuscript?: Research

\item 1. How relevant is this manuscript to the readers? Explain under Public Comments: Relevant

\item 1. Please explain how this manuscript advances this field of research and/or contributes something new to the literature.: In this work, the authors discuss a new method for detecting false data injection in networks of phasor measurement units. The authors argue that PMUs are susceptible to single-point data injection attacks which could compromise the stability of an electrical transmission or distribution network. The authors present three possible modes of attack: mirroring, repeated last value, and time dilation. They demonstrate how to detect these attack modes by comparing PMU readings in a local network. It appears that the technique of using large datasets coupled with machine learning is new in this body of work.

\item 2. Is the manuscript technically sound? Please explain your answer under Public Comments below.: Yes

\item 1. Are the title, abstract, and keywords appropriate? Please explain under Public Comments below.: Yes

\item 2. Does the manuscript contain sufficient and appropriate references? Please explain under Public Comments below.: References are sufficient and appropriate

\item 3. Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? Please explain your answer under Public Comments below.: Yes

\item 4. How would you rate the organization of the manuscript? Is it focused? Is the length appropriate for the topic? Please explain under Public Comments below.: Could be improved

\item  5. Please rate the readability of the manuscript. Explain your rating under Public Comments below.: Easy to read

\item 6. Should the supplemental material be included? (Click on the Supplementary Files icon to view files): No, it should not be included at all

\item 7. If yes to 6 (above), should it be accepted: After revisions.  Please include explanation under Public Comments below.
\end{itemize}

Please rate the manuscript. Explain your choice.: {\bf Good}


\subsection{Reviewer: 2}

Recommendation: {\em Author Should Prepare A Major Revision For A Second Review}

{\em Comments:}
In order to detect spoofing in PMU data, this paper uses machine learning techniques to inspect the correlation of data from nearby PMUs. Three possible spoofing strategies, Repeated-Last-Value, Mirroring, and Time-Dilation, are considered. Simulations are used to show the performance of the proposed detecting methods.

This paper does show a novel method to detect PMU data spoofing, while some key parts lack clear enough explanation. Here are the detailed concerns.

\begin{itemize}
\item The proposed method in this paper needs data from multiple PMU. Does other work also need data from multiple PMU? I have this concern because, if multiple PMU data are needed, then the detection algorithm can only run at the control center, i.e., in a centralized way. In contrast, if only local PMU data are needed, then the detection algorithm can run in a distributed way, which is more preferable.

\blue{We've further clarified that our system runs using data from multiple PMUs in the introduction and added text in the related work section to indicate that most other spoof detection systems share this requirement. } 

\item The second constraint in the first paragraph of Section IV.A is unclear. Does this constraint imply the monotonicity of $s(t)$ with respect to t? If so, then why the true signal must be monotone?

\blue{No, the second constraint indicates that: {\em ``the onset of a spoof should not create a discontinuity--that is, a signal $s$ sampled immediately before the spoof, $s(t-1) = s_{true}(t-1)$, and at the start of the spoof $s(t) = s_{spoof}(t)$, should show a change in value that is consistent with historical movement of that signal.''} This does not imply monotonicity of $s(t)$ with respect to $t$ either before or after the spoof. It simply requires that the step in two adjacent measurements should not itself give away the spoof.  That is, for any $k>=t$, $|s(k)-s({k-1})|$ should be selected from the range of values observable when $k<t$. Note also that we've changed the notation for the time series from $s_t$ to $s(t)$ with the aim of clarifying the points below.} 

\item In the fourth paragraph of section IV.A, please define the first derivative of $s(t)$ (note that t is discrete here). Do you mean something like $s(t)'=s(t)-s(t-1)$?

\blue{Correct.  We've updated the notation to make that clear.}

\item Please explain why only these three spoofing strategies (Repeated-Last-Value, Mirroring, and Time-Dilation) is considered. Do those strategies appear in other literature? Do they have advantages over other possible strategies?

\blue{These spoofing strategies do appear in other literature, we've clarified that in text. Their advantages are listed in Paragraph 1 of Part A in the Methodology section (IV.A)}

\item  The time-dilation spoof stated in the last paragraph of Section IV.A is quite unclear. Please define the concepts such as "cycles" and "play back" used in this paragraph. An example of this spoof is highly recommended for better illustration.

\blue{We've added additional description in Section IV.A as well as a graphical illustration of the time-dilation spoof.}
\end{itemize}

Additional Questions:
\begin{itemize}
    \item Which category describes this manuscript?: Technology

\end{itemize}

How relevant is this manuscript to the readers? Explain under Public Comments: Relevant
\begin{itemize}
\item 1. Please explain how this manuscript advances this field of research and/or contributes something new to the literature.: 1. Use correlation to detect spoofing.

\item 1. Apply machine learning to real PMU data streams.

\item 2. Is the manuscript technically sound? Please explain your answer under Public Comments below.: Partially

\item 1. Are the title, abstract, and keywords appropriate? Please explain under Public Comments below.: Yes

\item 2. Does the manuscript contain sufficient and appropriate references? Please explain under Public Comments below.: References are sufficient and appropriate

\item 3. Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? Please explain your answer under Public Comments below.: Yes

\item 4. How would you rate the organization of the manuscript? Is it focused? Is the length appropriate for the topic? Please explain under Public Comments below.: Satisfactory

\item 5. Please rate the readability of the manuscript. Explain your rating under Public Comments below.: Readable - but requires some effort to understand

\item 6. Should the supplemental material be included? (Click on the Supplementary Files icon to view files): Does not apply, no supplementary files included

\item 7. If yes to 6 (above), should it be accepted:
\end{itemize}

Please rate the manuscript. Explain your choice.: Good


\subsection{Reviewer: 3}

Recommendation: Revise and Resubmit as “New”

Comments:
\begin{itemize}
\item Page 1 - Space missing column 2 "The second dataset"
\item Page 2 - Space missing column 1 "Second, to the best..."
\item Page 2 - Spelling "withing"
\item Page 2 - Gramma "As noted previously, PMU data have..."
\item Section F. Common Limitations - what is H?
\end{itemize}
{\em Major concerns -}
\begin{enumerate}

\color{orange}
\item No mention of Ukraine and associated literature on the topic.

\color{blue}
We've added mention of the 2015 Ukraine attack, and a reference, to Section II: 
\\ \\
``Another example of using false data to facilitate a cyber attack was the multifaceted 2015 disruption of generation facilities in Ukraine~\cite{7752958}. Operators were prevented from sending commands to remote SCADA devices because the attackers had corrupted those devices with malicious firmware. This prevented operators from bringing generation resources back online after the initial attack.''

\color{orange}
\item No mention of the \$77 million DARPA program on topic and the supporting literature - looking at impedance estimation to identify an attack.

\color{blue}
ECS: I assume they are talking about RADICS projects here? I haven't seen much literature to come out of it yet, but here are some ideas to trace: 

Pal, Seemita, Biplab Sikdar, and Joe H. Chow. ``Classification and detection of PMU data manipulation attacks using transmission line parameters.'' IEEE Transactions on Smart Grid 9, no. 5 (2017): 5057-5066.
(This above is also the group working on distribution level PMUs so we could use the reference for both comments) 

Davis, Katherine R., Charles M. Davis, Saman A. Zonouz, Rakesh B. Bobba, Robin Berthier, Luis Garcia, and Peter W. Sauer. ''A cyber-physical modeling and assessment framework for power grid infrastructures.'' IEEE Transactions on smart grid 6, no. 5 (2015): 2464-2475.

This group was also looking at probing in terms of line impedance, but they started with this: 
Estimation of transmission line parameters from historical data
KR Davis, S Dutta, TJ Overbye, J Gronquist
2013 46th Hawaii International Conference on System Sciences, 2151-2160

\color{orange}
\item No mention of False Data Injection Attacks and the supporting literature on the topic.
In general, the literature referenced is focused on pre-2015 before the Ukraine cyber incident, after which considerable literature on the topic followed.
\\
\color{blue}

ECS: Adding some references here to discuss. Added to smartgrid2.bib as well,

brahma2016real
S. Brahma, R. Kavasseri, H. Cao, N. R. Chaudhuri, T. Alexopoulos, andY.  Cui,  “Real-time  identification  of  dynamic  events  in  power  systems using  pmu  data,  and  potential  applications—models,  promises,  and challenges,” IEEE  transactions  on  Power  Delivery,  vol.  32,  no.  1,  pp.294–301, 2016

Yasinzadeh2018detection
M.  Yasinzadeh  and  M.  Akhbari,  “Detection  of  pmu  spoofing  in  powergrid based on phasor measurement analysis,” IET Generation, Transmis-sion Distribution, vol. 12, no. 9, pp. 1980–1987, 2018.


\color{orange}
\item No mention is made on the accuracy of distribution-level PMUs and what level of accuracy is needed to measure distribution phase angles.

\color{blue}
We have found that the quality of the phase angle resolution is the same for distribution and transmission level PMU data, and both are sufficient for calculating the Pearson Correlation between PMU data streams. We have not had issues calculating phase angles from distribution-level PMUs, and as such, we don't discuss the issue within the manuscript.

\color{orange}
\item No mention of the relevance of the positive sequence for distribution circuits is made - especially given distribution grids are not often balanced and the circuits are not typically transposed.

\color{blue} The positive sequence exists in a three phase system regardless of system balance or transposition.  It is highly relevant, in both transmission and distribution, as it is the component that carries apparent power.  Consider too that at the point of measurement, the substation, distribution systems are relatively balanced.  Even along the lengths of feeders, the positive sequence component remains by far the largest of the sequence components, and is readily available for correlation with nearby PMUs. 
\\
Lack of transposition is just another source of imbalance, which, if significant, would be captured in the negative sequence component. However, distribution lines are usually too short to justify transposition.  We don't see this as an issue of concern.  The manuscript demonstrates that we are able to use correlation of positive sequence phase angle from distribution PMUs effectively.

\color{orange}
\item In Section Feature Extraction, a stronger justification for the correlation approach is needed

In section V.B. paragraph 4, we discuss the degree of correlation of PMU data parameters between PMUs.  We note that ``correlation vectors $r(|V_+|)$, $r(\phi_+)$ and $r(f)$ are good candidates for detecting spoofing attacks, as these consistently exhibit moderate to high correlation values over wide ranges of time. The $r(\phi_+)$ correlation values are exceptionally high, near 1.0 under normal circumstances.''  We outline our methods and demonstrate results in more detail in another publication, a citation to which has been added at the end of this paragraph.

\color{orange}
\item Section E. Evaluation Metrics - no mention of data quality is made - signal drop out is common with PMU data - how might this impact the results?

\color{blue}
A paragraph was added discussing data drop and data drift issues, which are common with PMUs.  We now include a reference to a study that demonstrated that drop and drift are easily detected through the Pearson Correlation method described in this paper.
\\ \\
``PMU data can be unreliable, and this lack of reliability can affect the aforementioned metrics.  For instance, a PMU may go offline, resulting in so-called ``data drop,'' which appears as a stream of zero-value data.  Other times, a PMU may produce the same measurements over a continuous period, often termed ``data drift.''  When processing PMU data for analysis, data drop and drift periods need to be removed.  Correlation can help.  As demonstrated by Meier et al., both data drop and data drift are easily identified through rapid decorrelation between the faulting PMU and near-by PMUs [Meier].''

\end{enumerate}

Additional Questions:
1. Which category describes this manuscript?: Practice / Application / Case Study / Experience Report

How relevant is this manuscript to the readers? Explain under Public Comments: Interesting - but not very relevant

1. Please explain how this manuscript advances this field of research and/or contributes something new to the literature.: I don't feel the manuscript advances the field in this research area.

2. Is the manuscript technically sound? Please explain your answer under Public Comments below.: Partially

\begin{itemize}
    \item 1. Are the title, abstract, and keywords appropriate? Please explain under Public Comments below.: No

\item 2. Does the manuscript contain sufficient and appropriate references? Please explain under Public Comments below.: Important references are missing; more references are needed

\item 3. Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? Please explain your answer under Public Comments below.: Yes

\item 4. How would you rate the organization of the manuscript? Is it focused? Is the length appropriate for the topic? Please explain under Public Comments below.: Could be improved

\item 5. Please rate the readability of the manuscript. Explain your rating under Public Comments below.: Easy to read

\item 6. Should the supplemental material be included? (Click on the Supplementary Files icon to view files): No, it should not be included at all

\item 7. If yes to 6 (above), should it be accepted: After revisions.  Please include explanation under Public Comments below.
\end{itemize}

Please rate the manuscript. Explain your choice.: {\em Fair}



==> PMU data/1_intro.tex <==
\section{Introduction} \label{sec:intro}

%\TODO{XZ}{PMUs, big data challenges, security concerns, data spoofs, application of machine learning techniques, prior work, contributions}

%\footnote{Do we need to cite BDCAT version? If so, where and how? ECS:~Yes. I believe in Section I, second to last paragraph, ``The contributions of this paper, building upon [BDCAT], are multifold...} 
Over the past decade, smart grid technology has become an emerging and fast-growing field within both research and industry. The fundamental concept of the smart grid is to enable and enhance wide-area monitoring, control and protection by leveraging advances in modern sensing, communication and information technologies. A core device of the smart grid is the phasor measurement unit (PMU), invented by Phadke and Thorp in the 1980s~\cite{1178427, Steinmetz1893, 5447627}. These devices provide near real-time measurements of Steinmetz's current and voltage phasors, which represent the real-time status of an electric grid. Measurements from widely-distributed geographical locations are synchronized with a precise clock using the global positioning system (GPS), providing each PMU data point with a precise time stamp aligned to a common time reference~\cite{schweitzer2010synchrophasor}. This time stamp allows PMU data from disparate locations to be synchronized, thereby providing a precise and comprehensive view of the entire grid.

Because of the enhanced monitoring capability enabled by PMUs, these devices have been widely adopted by electric utilities, balancing authorities, and transmission operators. From 2009 to 2014, PMU deployment in the U.S. increased from 200 PMUs~\cite{NERC14installation} to approximately 1700~\cite{clean14installation}. However, along with the value these devices bring to the power grid, they also introduce new challenges.
%in everyday operation of the grid. First of all, the 
The volume of data PMUs generate presents challenges for the traditional workflow of grid operations. Specifically, PMU sampling and recording rates range from 10-60 samples per second~\cite{1611105}. This is much higher than conventional monitoring technologies such as supervisory control and data acquisition (SCADA)~\cite{daneels1999scada}, which only sample once every two to four seconds. As a result, the volume of data to be stored, retrieved, processed, and analyzed is significantly larger than that of conventional systems. For instance, the Bonneville Power Administration's PMU network generates about 1.5 terabytes of data per month. This number is increasing as new PMUs are added to the system. 

Besides the big data challenges, data security and integrity are also critical concerns. Data integrity can be compromised due to various causes, such as data drops, clock drifts, or injection of deceptive data signals. If PMU data are used to inform power systems operations, these types of deterioration can affect control operations, ultimately leading to major problems such as cascading failures.

To address these challenges, research developed within the fields of big data analytics and machine learning can be applied to efficiently process and analyze PMU data, as well as detect any data disruption as it happens. In this paper, we present our work on evaluating two widely-used machine learning methods, Support Vector Machines (SVM) and Artificial Neural Networks (ANN), on detecting malicious data injections in PMU data streams. We use two datasets containing PMU data collected from real power systems. The first dataset, {\em BPA\_Data}, comes from PMUs within Bonneville Power Administration's 500 kV transmission network.% wide-area monitoring system in the U.S. Pacific Northwest. These PMUs are deployed on the 500 kV transmission network. 
The second dataset, {\em OSU\_Data}, was collected from the inter-university PMU network we built with three universities in the region: Washington State University in Vancouver, Portland State University, and Oregon State University and contains data from the distribution level. Using these two datasets, we conducted a comprehensive evaluation of the effectiveness of SVM and ANN in detecting spoofed signals within PMU data streams. 

The contributions of this paper are multifold. \oldblue{First, we have identified a set of features derived from historical PMU measurements, that can be used to reliably train both SVMs and ANNs to effectively identify spoofs without extensive parameter turning}.  \blue{Additionally, because our method identifies spoofs at the phasor data concentrator (using data from mutiple PMUs) it is immune to attacks that involve physical penetration of substations, individual pmus, or individual private network links.} Second,%\footnote{Review from this point to end of paragraph after new material is added}, 
to the best of our knowledge, this is the first comprehensive evaluation of multiple machine learning methods for spoof detection within PMU data streams. Third, we showed that the performance of training an ANN can be improved significantly by leveraging the techniques of distributed computing. This provides potential for future work in real-time detection of spoofed signals. And lastly, to the best of our knowledge, this paper is the first to apply machine methods to PMU data at both the transmission level and the distribution level. Our results show that SVM and ANN are effective for detecting spoofed data within datasets. We expect these results to demonstrate the value of using machine learning and data analytics techniques to solve engineering problems withing the electric power industry. 

The organization of the rest of the paper is as follows. In Section~\ref{sec:related}, we present related work in the cyber security aspect of the power grid, as well as applications of machine learning methods in this field. Section~\ref{sec:datasets} introduces the two datasets used in this study and discusses their  characteristics. In Section~\ref{sec:methodology}, we describe the methodology of our work, specifically for data processing, feature selection, and evaluation metrics. Section~\ref{sec:results} presents the evaluation results of both SVM and ANN, in terms of their performance in both detection, and training timespan. Finally, Section~\ref{sec:conclusion} concludes the paper and presents potential future directions for this work. 

==> PMU data/2_related.tex <==
\section{Related Work}\label{sec:related}

Cyber-security has long been a major concern for critical infrastructure, defined as assets essential for the functioning of a complex society~\cite{o2007critical}. Examples of critical infrastructure include electric power systems, natural gas and oil pipelines, and water supply systems. These facilities are monitored and controlled using Supervisory Control and Data Acquisition (SCADA) systems. SCADA systems collect measurement data from widely-distributed remote terminal units and issue control actions to the device-level layers within the infrastructure. 

\oldblue{Cyber-security incidents involving energy delivery systems} and associated theoretical attack structures are well documented~\cite{giani2009viking, miller2012survey, 7360168}. These attacks, sometimes intelligently designed and executed, are difficult to detect, especially when disguised via spoofing techniques. For instance, in 2010, Stuxnet~\cite{5772960, 6471059, 5742014}, a computer worm designed to infiltrate industrial equipment, altered the setpoint speed of centrifuges drives in an Iranian nuclear facility near Natanz, thereby causing the centrifuges to malfunction. During attacks, Stuxnet used spoofed data to mask malicious activities so that operators were not aware of the setpoint changes. Another example of using false data to facilitate a cyber attack was the multifaceted 2015 disruption of generation facilities in Ukraine~\cite{7752958}. Operators were prevented from sending commands to remote SCADA devices because the attackers had corrupted those devices with malicious firmware. This prevented operators from bringing generation resources back online after the initial attack. A third example is a series of cyber-attacks reported by McAfee in 2011 called `Night Dragon.' These attacks targeted global energy and oil firms, and exfiltrated critical data such as operational blueprints~\cite{nicholson2012scada}. These attacks had been ongoing for more than two years before they were identified because the attackers used a set of tools to compromise the target computers and mask their identity. 

\oldblue{Recently, with more information and networking technologies being integrated within smart grids, cyber security concerns in power systems now receive an increasing amount of attention. Because PMUs are critical data sources~\cite{pmu-wide-area-security, 780916}, these devices and their communication channels could become targets of cyber-physical attacks. Most PMUs in service are limited to providing data that informs intermediate algorithms, such as state estimation or voltage-stability assessment. %Such attacks are particularly unsettling when the target PMUs are not limited to serving as data sources to other intermediate algorithms such as state estimation or voltage-stability, but on the contrary, the PMU data are used for direct control of a protection system.  
The threat of cyber attack becomes unsettling when the target PMUs provide data for direct control of a protection system. For example, the Bonneville Power Administration pioneered the activation of Remedial Action Schemes (RAS) based on PMU data \cite{BPARAS18, 6672877, BPARASReport}.  A cyber attack on these PMUs would render the RAS inoperable.}

As noted previously, PMU data have GPS time stamps. Jian et al.~demonstrate this feature is a potential attack vulnerability~\cite{6451170}. Zhang et al.~examine the consequences of an attack on the time stamps of data collected within a smart grid wide-area network~\cite{Zhang2011}. Shepard et al.~surveyed and evaluated the vulnerabilities of PMUs to GPS spoofing attacks~\cite{Shepard2012}. Ng and Gao developed strategies to increase robustness of PMU time estimation~\cite{7479735}. Introduction of PMUs at the distribution level (aka micro-PMUs) allowed recent studies to identify attacks by coupling voltage and current data with network traffic data analysis \cite{tpwrs-dist,tsg-dist}. 

Within in the power systems community, PMU data spoofing outside of GPS signal manipulation has received attention for at least the last ten years. For example, detection of PMU data manipulation attacks by monitoring the impedances of transmission lines~\cite{8585968}. It has been shown in~\cite{Yasinzadeh2018detection} that phasor measurement analysis and state estimation methods can be combined to detect spoofed data. Real-time detection has also been addressed~\cite{brahma2016real}. 

%However, much of the previous work suffers from practical limitations in that: (1) it models spoof detection using dc power flow state estimators; and (2) assumes that the telemetry signals used for spoofing/detection only involve voltage magnitude and phase angle. As described in Section~\ref{sec:limitations-of-previous-work}, our method overcomes each of these issues. 

Compared with SCADA systems, PMUs provide sample data at a much higher rate, normally at 30, 60, or 120 samples per second, as opposed to traditional SCADA refresh rate of seconds or even minutes. As a result, the amount of data generated by PMUs is significantly larger than that of a SCADA-based system. Therefore, big data challenges, in particular for online applications~\cite{streamcast2018} are inevitably introduced to these systems. To address these challenges, big data and machine learning techniques may be leveraged and applied to PMU data storage and processing. A variety of machine learning techniques have been applied to analyze PMU data for the purpose of recognizing patterns or signatures of events. Both \textit{classification}~\cite{nguyen2015smart} and \textit{clustering}~\cite{eric-smartgreens16} are effective methods in analyzing PMU data streams for event detection. And, \textit{one-class learning} has the potential to identify anomalies in PMU data~\cite{wallace-bigdata16}. Machine learning techniques have proven effective at detecting security attacks in cyber-physical systems, including electric power systems~\cite{mitchell2013effect, amor2004naive, kher2012detection}. \oldblue{However, none of these approaches have been evaluated on PMU data from a functioning power system.}

\blue{The majority of prior work examining spoof detection on PMU signals are similar to ours in that they are designed to run at a central datacenter with access to multiple sensor/PMU signals (e.g., ~\cite{6740901,landfordfast,kher2012detection,Ma20}). The benefit of this approach is that intruders cannot evade detection by injecting their spoof upstream of the detector. This means that any physical attack against the substation, its PMUs or the network connecting the substation to the data center are defended.  Further, although our approach cannot run at the edge of the network (e.g., at an individual PMU), it is does not need full observations from {\em all} PMUs. Instead, it is designed to run on a small subset of PMU signals which improves scalability as the number of PMUs increase and allows the algorithm to run before all PMU signals have been aggregated.} 

The work presented here is distinguished in the following ways. First, \oldblue{spoofs are identified by observing changes in PMU signal correlation between pairs of PMUs}~\cite{landfordfast}. Magiera and Katulski used a similar approach for spoof detection, though focused on Global Navigation Satellite Systems signals instead of PMU data~\cite{6614026}. Second, to the best of our knowledge, no previous work has evaluated machine learning methods using real PMU data streams at both the transmission and distribution levels. %This paper presents our work in this direction. 
Third, our method explicitly considers, and avoids, the two limitations from previous work on detecting PMU spoofs identified above. Finally, we demonstrate the potential for achieving more efficient training performance by leveraging a distributed computing framework. This is the critical initial step to apply these methods to real-time PMU data streams for online spoof detection, which has not been addressed in previous literature. 


==> PMU data/3_dataset.tex <==
\section{Datasets}\label{sec:datasets}

%\TODO{XZ}{Transmission level and distribution level datasets}

%A smart grid structure and our data collection method are shown in Figure~\ref{fig:datasets}. The structure of an electric power grid is composed of four main components: generation, transmission, distribution, and consumers. These components represent the basic workflow of a power grid. Generation refers to various power plants that generate power. The transmission network consists power lines and substations responsible for transmitting the electricity from its place of generation to the distribution level. These lines and substations operate at a high voltage level (e.g., 500 kV), in order to minimize large voltage drops and $I^{2}R$ losses within transmission line conductors. The distribution network represents the final stage in the delivery of electric power, distributing electricity from the transmission system to individual consumers. Distribution substations convert high voltage power from the transmission system to a medium-range voltage for distribution (under 100kV) using step-down transformers. Primary distribution lines carry this medium voltage power to distribution transformers located near customer premises. Distribution transformers lower the voltage further to utilization voltages used by lighting, industrial equipment and household appliances. 

Within an electrical grid, PMUs may be deployed at both the transmission and distribution levels to enhance situational awareness. These devices, as well as their communications network, may be targets of a cyber attack. In order to develop an effective approach for detecting such attacks, it is essential to evaluate at both the transmission level and the distribution level. Therefore, we have collected and analyzed PMU data from both levels for this study; dataset {\em BPA\_Data} came from a transmission network, while dataset {\em OSU\_Data} came from a distribution network. 
%As illustrated in Figure~\ref{fig:datasets}, {\em BPA\_Data} came from a transmission network, and {\em OSU\_Data} came from a distribution network. 

%\blue{remove Fig ?1}

%\begin{figure}[h]
%    %\centering
%    \includegraphics[width=0.45\textwidth]{figs/datasets.pdf}
%    \caption{Data Collection on the Smart Grid}
%    \label{fig:datasets}
%\end{figure}

\subsection{Transmission Level Dataset}

{\em BPA\_Data} was provided by Bonneville Power Administration, one of the first transmission operators to implement a comprehensive adoption of synchrophasors within a wide-area monitoring system. This dataset contains data collected by ten PMUs within BPA's 500 kV PMU network. Note that there are more PMUs deployed in BPA's transmission network. We chose to use ten PMUs for the following reasons. First, based on historical cyber-security incidents, these attacks usually have one specific target, either a device or a network channel. Therefore, to mimic these attacks and evaluate the spoof detection approaches, using data from a small set of PMUs is sufficient. Second, being able to detect cyber attacks using only local information from nearby PMUs is critical. This enables efficient detection. The same approach can be deployed to cover the whole system using a divide-and-conquer approach. The ten PMUs selected for this study are electrically-close to each other, based on their \textit{electrical distance}, which has been shown to be a useful representation of power system connectivity~\cite{hines2010topological}. Third, selecting 10 PMUs keeps the dataset at the same scale as our distribution level dataset, for the purpose of comparison. 

\subsection{Distribution Level Dataset}

{\em OSU\_Data} comes from seven PMUs from our research-grade, inter-university PMU network. This dataset provides PMU data samples from the distribution level. Our research PMU network consists of seven PMUs, one each at the Washington State University-Vancouver (WSU-V) and Portland State University (PSU) campuses, with the remaining five placed at multiple locations across the Oregon State University (OSU) campus. The PMUs provide monitoring at the utilization level (120/208 V), with the exception of two PMUs at OSU, which monitor a 4 kV and a 20 kV distribution substation. All PMUs monitor three phase services. 

In our distribution level PMU network, all the PMUs report data at 60 samples per second to a Phasor Data Concentrator (PDC) located at the OSU campus. The data management scheme on the PDC emulates real PDC setups. A local archive stores 60 days of data on the PDC. The files are archived to  another server for permanent storage. %\green{\st{In addition to using commercially-available software from SEL, which stores data in .csv and SynchroWAVe formats, the PDC uses PDAT recording software.% that is currently deployed at Bonneville Power Administration. All of these file-types are archived for permanent storage so that we may reliably access them from a variety of software tools.}}\footnote{SW: I think we can cut this (ditto all green strike through)}

% I (RB) don't think we need this paragraph and table -------------------------------------------------------->>>

%These two datasets provide data from both the transmission level and the distribution-level. Using these dataset, we can evaluate spoof detection techniques in a comprehensive manner. The main characteristics and collection dates of both datasets are summarized in Table~\ref{tab:datasets}. 

%\begin{table}[h]
%    \centering
%    \caption{Characteristics of Datasets}
%    \begin{tabular}{|c|c|c|c|}
%    \hline
%        {\bf Dataset} & {\bf Type} & {\bf \# PMUs} & {\bf Date Collected} \\
%        \hline
%        BPA\_Data & Transmission & 10 & 2013-06-26\\
%        \hline
%        OSU\_Data & Distribution & 7 & 2017-06-03\\
%        \hline
%    \end{tabular}
%    \label{tab:datasets}
%\end{table}

% -----------------------------------------------------------------------------------------------<<<<


==> PMU data/4_methodology.tex <==
\section{Methodology}\label{sec:methodology}

%\TODO{XZ}{Spoofing strategy, Features, methods, evaluation metrics, experimental design, experimental environment}

One lesson learned from major cyber-security incidents, including Stuxnet and Night Dragon, is that attackers often mask their malicious activities via spoofing. In other words, they inject spoofed signals into the system to disguise cyber attacks. These spoofed signals are designed in a way that the system cannot easily identify the data as falsified.  %\green{\st{This presents an additional challenge for detecting the underlying attacks.}} 
\oldblue{However, given that the falsified data is not an accurate measurement of the system state, there are limits in power systems to how well a spoof can be disguised}. %\green{\st{To mimic these effects,}}
We developed three strategies for generating spoofed signals. In this section, we present these strategies, our methods for feature extraction, two machine learning techniques, and our evaluation metrics. 

\subsection{Spoofing Strategies}

%\green{\st{Data spoofing is often used in cyber attacks to mask malicious activities. Sophisticated spoofs are similar to normal data, making it difficult for the system or operators to identify attacks. Previous work has been done to mimic this effect and develop various spoofing strategies for PMU data streams}}~\cite{landfordfast}.

%\begin{figure}[h]
%    %\centering
%    \subfigure[Original Signal]{\includegraphics[width=0.45\textwidth]{figs/raw.png}\label{fig:spoof_before}}
%    \subfigure[Spoofed Signal]{\includegraphics[width=0.45\textwidth]{figs/mirrored.png}\label{fig:spoof_after}}
%    \caption{Data Spoofing Strategy: Mirroring}
%    \label{fig:spoof}
%\end{figure}

\blue{To describe our spoofing strategies, we use the following notation. A signal measured at time step $k$ is denoted $s(k)$. If a spoof begins at time step $t$, then $s(k) = s_{true}(k)$ for $k < t$ and $s(k) = s_{spoof}(k)$ for $k >= t$. That is, prior to $t$ the measured signal is exactly the true signal, otherwise the signal is provided by some spoofing method.} 

\blue{Our spoofing strategies aim to prevent easy detection and are designed in consideration of the following constraints: (1) spoofs should provide historically-reasonable values for the target signals; (2) the onset of a spoof should not create a discontinuity---that is, a signal, $s$, sampled immediately before the spoof, $s(t-1) = s_{true}(t-1)$, and at the start of the spoof, $s(t) = s_{spoof}(t)$, should show a change in value that is consistent with historical variation of that signal; (3) spoofed data should only require knowledge of the local signals, and not, for example, knowledge of signals at other PMUs. Below, \blue{we describe the three strategies employed for this study for generating $s_{spoof}$. These strategies all meet the criteria above and have been explored in prior work (e.g., \cite{jiang00fault,Ma20})}: {\em Repeated-Last-Value}, {\em Mirroring} and {\em Time-Dilation}.} 

\oldblue{The {\em Repeated-Last-Value} (RLV) spoof represents the strategy consistent with the constraints outlined above. This spoof requires knowledge of the true signal values immediately prior to the spoof onset, and repeats these values for the duration of the spoof. \blue{That is, assuming a spoof begins at time $t$, the signal $s(t+i) = s_{spoof}(t+i) = s_{true}(t-1)$ for all $i>0$}.}

% work, we use the {\em Mirroring} spoof strategy. Specifically, the spoofing was derived by recording 90 seconds (5400 cycles) of PMU data from one of the PMUs in our datasets, then playing back these data in reverse to generate spoofed signal for 90 seconds, to mask the real data in this time period. Figure~\ref{fig:spoof} shows the effect of the mirroring spoof. Here, we show the voltage magnitude signal measured by one of the PMUs at OSU, namely SNELL, in a 5-minute window. Figure~\ref{fig:spoof_before} shows the original data stream we collected. The red dotted line indicates the 90th second in time, i.e., 5400 cycles, where the spoofed signal will be injected.\footnote{Here, we choose the 90th second as the injection time, just for illustration purpose. In the later experiments, we spoof 30 seconds of data.} Figure~\ref{fig:spoof_after} shows the signal after the mirroring spoof has been applied. The signal on the right side of the dotted line is replaced by the spoofed signal, i.e., a reverse replay of the data in the first 90 seconds. Note that replaying the signal in reverse guarantees signal continuity for all parameters at the instance spoofing is initiated.

\oldblue{The main short-coming of the RLV spoof is that it provides a constant value signal. Although the signal can clearly be guaranteed to remain within historic range, and will produce no discontinuity at the spoof onset, the distribution of values during the spoofed period will clearly be abnormal.} 

\oldblue{The {\em Mirroring} spoof improves upon the shortcoming of the RLV. To stage this attack, the adversary records the target signal for a period of time $u$ prior to the spoof, and then when the spoof begins at time $t$, \blue{sets $s(t+i) = s_{spoof}(t+i) = s_{true}(t-i)$ for $i=0\dots u$. However, mirroring imposes an immediate sign change on the signal's first derivative ($s(t) - s(t-1) = -s(t+1) + s(t)$).} Thus, mirroring produces an inflection point in the signal data when the spoof begins, violating our second constraint. } 

%The mirroring spoof is a simple but powerful spoofing strategy. The spoof is derived from the real signal, carrying the same characteristics, such as noise level, frequency, etc. The high similarity between real signal and the spoofed signal presents challenges for the spoof detection methods. In addition, the mirroring spoof is easy to calculate, and since it is only based on an historic data stream, it is possible to generate as much spoofing as needed to mask the real data. The mirroring spoof is used in our work to evaluate the spoof detection approaches. Specifically, we perform mirroring spoofing on one of the PMUs in each datasets and use the spoofed data to evaluate the effectiveness of each approach in accurately detecting the spoofed signals. 

\oldblue{The {\em Time-Dilation} spoof plays recorded data back at a slower than normal rate. A time dilation of $2x$ records data for $n$ \blue{time steps (cycles)}, but plays these back over $2n$ cycles. Like mirroring, time-dilation upholds the three constraints while providing a historically-reasonable distribution of signal values. Unlike mirroring, however, time-dilation also improves continuity of the signals' first derivative. Time-dilation preserves the sign of the signal's derivative, but impacts the derivative's magnitude proportionally to the amount of dilation. In addition, unlike RLV and Mirroring, which provide an immediate window for malicious action when the spoof begins, time-dilation requires that the attacker continues to monitor, record, and resample live signal data even as the spoof begins. As a result, the attacker's window for malicious action occurs sometime after the spoof has begun, instead of at the onset.}

\blue{Figure~\ref{fig:2xdilation_spoof} illustrates the spoof; the true signal is plotted as a dashed line, the spoof as a solid line. The spoof begins at cycle 250, illustrated in the plot by the fact that the solid line begins to diverge from the dashed line at this point. From cycle 250 forward, $s(t) = s_{spoof}(t) = s_{true}( 250 + (t-250)/2 )$. Thus, to perform the spoof, the true signal must be recorded for some portion of time after the spoof begins. That is, in this illustration, the true signal has been recorded from cycles 250 through 1125 and that waveform is played back between cycles 250 and 2000.} 

\blue{It should be noted that for this spoof, and all other spoofs described above, our focus is on the spoof onset. That is, we are interested in detecting the spoof as early as possible.  Our spoofs are generated on the last 30 seconds of a one minute sample and we make no attempt to force the spoof and the true signal to re-align once the spoof is complete.  This experimental setup strongly favors the spoofer by assuming that any discontinuity created at the end of the spoof between the last cycle of the spoofed data and the first cycle of real signal post-spoof (e.g., in Figure~\ref{fig:2xdilation_spoof} between the spoofed signal at cycle 2000 and whatever comes next) cannot be detected.}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figs/2x_dilation.pdf}
    \caption{2x dilation spoof}
    \label{fig:2xdilation_spoof}
\end{figure}    

%\footnote{this seems a bit confusing, either we could remove this, or add more discussion and perhaps a picture}\footnote{I think it is well-written. RB}.





We designed our spoof strategies, e.g., mirror, time dilation etc., using real PMU data to demonstrate the effectivenss of our detection algorithm. A spoof that is created using real high-resolution PMU data is harder to detect. If the attacker does not have the real PMU data, it is easier for the algorithm to detect the spoof. 



\subsection{Feature Extraction} \label{sec:feature}

% Target for potential space savings:
Feature extraction is a critical step in applying machine learning techniques to solve a problem. When performing analysis of complex data, one of the major problems stems from the number of variables/features involved. Analysis with a large number of variables generally requires a large amount of memory and computation power. Also, it may cause a classification algorithm to overfit to training samples and generalize poorly to new samples. Feature extraction aims for constructing combinations of the features while still describing the data with sufficient accuracy. In our work, one of the main objectives is to develop a generic set of features from PMU data that can be used by multiple machine learning algorithms for detecting spoofed signals.%\footnote{SW: this paragraph could be reduced by half} 

PMUs measure phasors of line voltages and line currents for all voltages (A, B, C) and currents (A, B, C, N).  From these are derived a number of other parameters, including magnitude and phase angle for the positive, negative and zero sequence voltages and currents; frequency; and, rate of change of frequency ($ROCOF$); among others~\cite{1611105}. In \cite{landfordfast}, we describe how intra-PMU parameters (i.e., correlation between different signals from the same PMU) are usually weakly correlated, yet the inter-PMU parameters (i.e., the same signal from different PMUs) are often highly correlated, especially when the PMUs are electrically close to each other, as would be expect from an electrical network featuring a range of electrical distances between nodes~\cite{Paper031}. These observations indicate that the correlations between PMU signals have great potential to serve as features to construct the models in machine learning techniques.%\footnote{SW: this could be spelled out a bit more here}. 

%To quantify the degree of correlation between PMU parameters, we use {\em Pearson Correlation Coefficient (PCC)} as the metric. The PCC of two data streams $X(x_1, x_2, ..., x_n)$ and $Y(y_1, y_2, ..., y_n)$ can be calculated as shown in Equation~\ref{equ:pcc}. 

%\oldblue{remove Equ 1}

%\begin{equation}
%\label{equ:pcc}
%PCC = \frac{\sum^{n}_{i=1}{(x_i-\overline{X})(y_i-\overline{Y})}}{\sqrt{\sum^{n}_{i=1}{(x_i-\overline{X})^2}}\sqrt{\sum^{n}_{i=1}{(y_i-\overline{Y})^2}}}
%\end{equation}

To quantify the degree of correlation between PMU parameters, we calculate the {\em Pearson Correlation Coefficient (PCC)} between two data streams, $X(x_1, x_2, ..., x_n)$ and $Y(y_1, y_2, ..., y_n)$.  Specifically, given PMUs numbered $1,2\dots ,p$ we develop ${p \choose 2}$ vectors of correlation values between a specific signal for every pair of PMUs $i < j$. This is repeated for eight signals: positive sequence voltage magnitude $|V_+|$, negative sequence voltage magnitude $|V_-|$, zero sequence voltage magnitude $|V_0|$, positive sequence phase angle $\phi_+$, negative sequence phase angle $\phi_-$, zero sequence phase angle $\phi_0$, frequency $f$, and $ROCOF$. 

After carefully examining the correlation data for these eight signals in a previous study, we made the following observations~\cite{landfordfast}. First, correlation vectors $r(|V_+|)$, $r(\phi_+)$ and $r(f)$ are good candidates for detecting spoofing attacks, as these consistently exhibit moderate to high correlation values over wide ranges of time. The $r(\phi_+)$ correlation values are exceptionally high, near 1.0 under normal circumstances. Second, $ROCOF$ correlation between PMUs is very poor, likely due to the fact that it is the second derivative of the positive sequence phase angle, and hence more susceptible to noise. Third, correlations on other signals, including $r(|V_-|)$, $r(|V_0|)$, $r(\phi_-)$ and $r(\phi_0)$, do not exhibit consistent moderate correlation. %Therefore, they may or may not add value to the learning process. 

Based on our observations, we chose five correlation features to use in the machine learning techniques. These include the three strongly correlated features, $r(|V_+|)$, $r(\phi_+)$ and $r(f)$, and two moderately correlated features, $r(\phi_-)$ and $r(\phi_0)$. These features are used in different learning algorithms to evaluate their effectiveness. Note that these correlation values fluctuate with time since the correlation is performed using data windows of a fixed length. In this work, we chose a fixed window of 5-seconds (300 cycles). 

%positive sequence voltage magnitude $R_{ij}(|V_+|)$ for every pair of PMUs $i < j$. This is repeated for the $|V_-|$, $|V_0|$, $\phi_+$, $\phi_-$, $\phi_0$, $f$ and $ROCOF$ data. These correlation values fluctuate with time, since the correlation is performed using data windows of a fixed length.

\subsection{Parallel Data Preprocessing}

\oldblue{The correlation features derived from the raw PMU data stream must be computed prior to training and then on a continuing basis during deployment. As a result, the cost of extracting features from the raw data has a real impact on computational resources that need to be continually dedicated to a tool such as this.}

%\oldblue{Although computing the signal correlations is an embarrassingly parallizeable task, the number of correlations that need to be computed grows quadratically in relation to the number of nearby PMUs. Thus, the constant factors associated with the preprocessing are relevant for determining real-world scalability.}

\oldblue{Computing the signal correlations is a parallizeable task, though the number of correlations that need to be computed grows quadratically in relation to the number of nearby PMUs. Thus, the constant factors associated with the preprocessing are relevant for determining real-world scalability.}

\oldblue{We compared the cost of a data preprocessing pipeline built using two common Python frameworks for parallel/distributed processing: Celery\cite{CeleryPython} and ipyparallel\cite{IPython}. Our results suggest that while inter-process queueing with Celery can add a significant performance penalty to parallelizing the feature extraction, the same is not true for ipyparallel.} 

\oldblue{With ipyparallel, we were able to scale feature extraction linearly with the number of correlation values and number of CPUs. Computing the correlations on a sliding 300 cycle window over 1 minute of data required 1.85 seconds of CPU time and scaled linearly up to 24 cores at which time computation became I/O limited on our system. This speed is well within realtime requirements: 10 PMUs each with 5 signals yields 225 correlations and requires 8 CPU cores to complete in real-time.}


Note that these preprecessing experiments are based on continuously calculating correlations using a 300-cycle sliding window with a step of 1 cycle. In reality, the sliding window can be adjusted by using larger steps, representing a trade off between the granularity of the correlations and the computational performance. Also, our previous study shows that for the spoof detection purposes, it is not necessary to calculate correlations for all PMU pairs, because a small number of PMUs that are electrically close to the spoofed PMU will be enough for the algorithm to trigger the detection. Therefore, the scalability issues can be addressed for a larger PMU network. 



%\begin{figure}[h]
%\centering
%\includegraphics[width=0.95\columnwidth]{figs/Preprocessing.pdf}
%\caption{Cost of Feature Extraction}
%\label{fig:feature_extraction_cost}
%\end{figure}

\subsection{Machine Learning Techniques}

Using the correlation features we derived from the raw PMU data streams, we carried out a comprehensive evaluation of two widely-used machine learning techniques, Support Vector Machine (SVM)~\cite{cortes95}, and Artificial Neural Networks (ANN)~\cite{yegnanarayana2009artificial}. 

An SVM is supervised learning model with associated learning algorithms that analyzes data for classification and regression analysis. Given a set of training examples, each marked as belonging to one or the other of two categories, an SVM training algorithm builds a model that assigns new examples to one category or the other, making it a non-probabilistic binary classifier. Specifically, an SVM model is a representation of the examples as points in space, mapped so that the examples of the separate categories are divided by a clear margin that is as wide as possible. New examples are then mapped into that same space and predicted to belong to a category based on which side of the margin they fall. Here in our case, we use the two-class SVM to learn a relationship that differentiates spoofed PMU signals from the normal  signals. We leverage the Python library \textit{sci-kit learn} for an SVM implementation based on libsvm~\cite{scikitlearn,libsvm}. 

Similar to the SVM, an ANN is another widely-used technique for supervised learning. It is a machine learning model inspired by the biological nervous system. This technique has been widely applied in the fields of computer vision, speech recognition, anomaly detection, etc. However, to the best of our knowledge, it has not been evaluated using power systems data in the context of spoof detection. 

An ANN is based on a collection of connected units called artificial neurons. Each connection (synapse) between neurons can transmit a signal to another neuron. The receiving (postsynaptic) neuron can process the signal and then send it to the downstream neurons connected to it. Neurons have a state, generally represented by real numbers, typically between 0 and 1. Neurons and synapses also have a weight that varies as learning proceeds, which can increase or decrease the strength of the signal that it sends downstream. Further, they \oldblue{have an activation function that determines how the aggregate input signals trigger an output signal.}

Typically, neurons are organized in layers. Layers are made up of a number of interconnected neurons which contain an activation function. Data features are presented to the network via the input layer, which communicates to one or more hidden layers where the actual processing is done via a system of weighted connections. The hidden layers then link to an output layer where the results of the learning are made available to the users. In our work, we built an ANN which has two hidden layers, each with 100 neurons. %Activation functions in hidden layers are both \textit{TanH}, which computes hyperbolic tangent\footnote{RB: more to this sentence...?}. The activation function of the output layer is \textit{Softmax}, which computes softmax activations.\footnote{RB: Do we need these last two sentences? Perhaps to much into the weeds for an EE publication.} 

\subsection{Evaluation Metrics} \label{sec:metrics}

To evaluate the effectiveness of the two machine learning techniques on detecting spoofed signals in PMU data, we carried out a number of experiments and took measurements on multiple metrics. Below, we describe the performance metrics we use in this study: 

\begin{itemize}[leftmargin=*]

\item[] \textbf{Accuracy}: %\green{\st{measures a classifier's performance over all examples in terms of identifying examples correctly. It}} 
is calculated as the number of correct predictions, i.e., true positives (normal examples identified as such) plus true negatives (spoofed examples identified as such), divided by the total number of examples. Accuracy ranges from $0\%$ to $100\%$ with an ideal classifier measuring $100\%$.

\item[] {\bf Sensitivity}: measures the ability to correctly detect spoofed signals, and is calculated as the number of true positives (spoofed examples identified as such) divided by the number of total positives (the total number of spoofed examples which is the sum of true positives and false negatives). Sensitivity ranges from $0\%$ to $100\%$ with an ideal classifier measuring $100\%$.

\item[] {\bf Precision:} measures how many of the positively classified were relevant and is calculated as the number of true positives (spoofed examples identified as such) divided by the number of detected spoofs (false positives plus true positives). Precision ranges from $0\%$ to $100\%$ with an ideal classifier measuring $100\%$.

\item[] {\bf Specificity:} measures the ability to correctly identify normal signals. It is calculated as the number of true negatives (normal examples identified as such) divided by the number of total negatives (the total number of normal examples which is the sum of true negatives and false positives). Specificity ranges from $0\%$ to $100\%$ with an ideal classifier measuring $100\%$.

\item[] {\bf F1:} measures performance as a single value when classes are not equally prevalent. It is the harmonic mean of Sensitivity and Precision. Scores range from 0.0 to 1.0; higher values are better.

\item[] {\bf False Discovery Rate (FDR):} measures the propensity to spuriously identify a spoof. This value is calculated as the number of false positives (normal examples identified as spoofs) divided by the number of detected spoofs (false positives plus true positives). False Discovery Rate is equivalent to (1-Precision). FDR ranges from $0\%$ to $100\%$; an ideal classifier has $0\%$ FDR.

\item[] \oldblue{{\bf Latency:} measures how long it takes to identify that a spoof is occurring. Recall that all the input features are signal correlation values calculated on a 5-second (300 cycle) window. Assuming a spoof begins at time $t$, the correlation value at time $t$ contains one spoofed value and 299 non-spoofed values. The correlation value at time $t+299$ is built from a window of entirely spoofed data. Our latency calculation measures how many cycles must occur before the classifier begins to consistently identify the spoof (marked by a contiguous set of thirty positive classifications). Thus, a latency of $0$ indicates that as soon as the correlation window contains one spoofed data element the classifier will subsequently detect $\ge 30$ consecutive cycles of spoofs.}

\end{itemize}


PMU data can be unreliable, and this lack of reliability can affect the aforementioned metrics.  For instance, a PMU may go offline, resulting in so-called ``data drop,'' which appears as a stream of zero-value data.  Other times, a PMU may produce the same measurements over a continuous period, often termed ``data drift.''  When processing PMU data for analysis, data drop and drift periods need to be removed.  Correlation can help.  As demonstrated by Meier et al., both data drop and data drift are easily identified through rapid decorrelation between the faulting PMU and near-by PMUs~\cite{UsSusTech14BPAEE}.


\subsection{Common Limitations}
\label{sec:limitations-of-previous-work}

\oldblue{As noted in Section~\ref{sec:related},  much of the previous work suffers from practical limitations in that: (1) it models spoof detection using dc power flow state estimators; and (2) assumes that the only telemetry signals involved in spoofing/detection are voltage magnitude and phase angle. Below we describe each of these limitations in more detail and describe how our methodology avoids these issues.}

\oldblue{First, as noted by Liu and Lie, most research on state estimation attacks use dc power flow models for \textbf{H}, whereas utility state estimators use ac models\cite{6740901}. In essence, this means that much of the earlier work on spoof detection makes assumptions that are invalid in practice. Linearized state estimators neglect reactive power flow, which has a significant impact on bus voltage magnitudes. Moreover, a state estimator using an ac \textbf{H} will produce large residues when subjected to attack vectors derived from a dc \textbf{H}. 
Our methods do not depend on a explicit system model \textbf{H}. Instead, an implicit model is captured by the learning algorithms in the course of analyzing historical time-series data. In our approach, correlation of physical phenomena at multiple measurement points would need to be known in order to construct an undetectable attack vector. This is a significant hurdle for attackers. That is, even if the attacker used an accurate and complete ac \textbf{H} to derive an attack vector, the correlation of state measurements would still collapse as soon as the false data are injected into the measurements. }

\oldblue{Second, both dc- and ac-based state estimators only use positive sequence voltage magnitudes and phase angles; no consideration is given to other data, such as negative and zero sequence voltages, frequency, or $ROCOF$, which are also calculated by PMUs. In contrast, to defeat a classifier built using the approaches we describe, an attacker would need to compromise \textit{and} correlate \textit{all} of the PMU data streams, not just $|V_{+}|$ and $\phi_{+}$. This means that our detection approach, which works outside of the state-estimation process, should be less susceptible to spoofing than a system that works as part of the state-estimation.
}



==> PMU data/5_results.tex <==
\section{Performance Evaluation}\label{sec:results}

Experiments have been carried out using both the BPA and OSU datasets to evaluate the effectiveness of SVM and ANN in terms of detecting spoofed signals. In addition, we also investigated the potential of distributing the training task to increase the computational performance. In this section, we present the process of preparing training and testing datasets, as well as the experimental results. 

\subsection{Training and Testing Data}

For both the BPA and OSU datasets, we prepare the training and testing examples as follows. First, we choose 14 independent minutes of normal data from the dataset. We then apply one of the spoof procedures (Repeated-Last-Value, Mirroring, and Time-Dilation) to the last 30 seconds of one selected PMU signal on each of 14 different minutes of data. Finally, we calculate the pair-wise correlation features, as described in Section~\ref{sec:feature}. For each spoof procedure, this approach generates roughly $2\cdot 10^6$ examples from the 14 minutes of data and the 45 PMU pairs (i.e., 10 PMUs) in the BPA dataset, and roughly $1\cdot10^6$ examples from the 14 minutes of data and the 21 PMU pairs (i.e., 7 PMUs) in the OSU dataset. Examples are ``Spoofed'' in the last half of each minute if $i$ is the spoofed PMU, and are ``Normal'' otherwise. Given the 14 minutes of data, we use 11 minutes (roughly $1.6\cdot10^6$ examples for BPA data and $8\cdot10^5$ examples for OSU data) for training, and 3 minutes (roughly $4.5\cdot10^5$ examples for BPA data and roughly $2.1\cdot10^5$ examples for OSU data) for testing. During training, all correlations features are standardized (normalized to 0 mean and standard deviation of 1). The normalization transforms from the training features are saved so they can later be used to transform testing data prior to being classified. Note that for the parameter selection in SVM, we have performed a grid search as follows. We first split the 11 training minutes into two sets (8 and 3 minutes respectively) and performed a grid search over the $C,\gamma$ parameter space by training on the former set and testing on the later. We observed high performance (F1 $>$ .95) across a wide range of parameter settings for both datsets. Thus, in subsequent sections, our results are obtained using the same set of parameters, $C=1.0$, $\gamma=0.2$. 

\subsection{Spoof Detection Performance}

For each of the spoof procedures, we train a two-class SVM and an ANN using 11 minutes of data, and then test its detection performance using the other 3 minutes of data. For each experiment, we measure the performance metrics described in Section~\ref{sec:metrics}. \oldblue{The experimental results for the three spoof procedures, i.e., RLV, Mirroring, and Time Dilation, are shown in Table~\ref{tab:RLV_new}, \ref{tab:mirror_new}, and \ref{tab:dilation_new}, respectively. }%\footnote{XZ: Add explanation about old- new-normalization?}

%The results for each experiment are shown in Figure~\ref{fig:detectionP} and Table~\ref{tab:detectionP}. 


%\begin{figure}[h]
    %\centering
%    \includegraphics[width=0.45\textwidth]{figs/bar_plot_with_FDR.png}
%    \caption{Spoof Detection Performance Comparison}
%    \label{fig:detectionP}
%\end{figure}

%\begin{table}[h]
%    \centering
%    \begin{tabular}{|c|c|c|c|c|}
%    \hline
%      {\bf Metrics}   & {\bf SVM\_BPA} & {\bf NN\_BPA} & {\bf SVM\_OSU} & {\bf NN\_OSU} \\
%      \hline
%        Accuracy &98.21\%  &98.47\% &94.07\% &94.24\% \\
%        \hline
%        Sensitivity    &83.75\%  &86.38\% &75.21\% &72.24\% \\
%        \hline
%        Precision   &99.74\%  &99.54\% &90.56\% &94.84\% \\
%        \hline
%        Specificity     &99.97\%  &99.95\% &98.26\% &99.13\% \\
%       \hline
%        F1    &0.911  &0.925 &0.822 &0.820 \\
%        \hline
%        FDR   &0.26\%  &0.46\% &9.44\% &5.16\% \\
%        \hline
%    \end{tabular}
%    \caption{Spoof Detection Performance Comparison}
%    \label{tab:detectionP}
%\end{table}


\begin{table}[h]
    \centering
    \footnotesize
    \caption{Spoof Detection Performance (RLV)}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
      {\bf Metrics}   & {\bf SVM\_BPA} & {\bf NN\_BPA} & {\bf SVM\_OSU} & {\bf NN\_OSU} \\
      \hline
        Accuracy &99.90\%  &99.97\% &99.05\% &99.26\% \\
        \hline
        Sensitivity    &99.13\%  &99.76\% &94.99\% &96.16\% \\
        \hline
        Precision   &99.96\%  &100.00\% &99.75\% &99.74\% \\
        \hline
        Specificity     &99.99\%  &100.00\% &99.95\% &99.94\% \\
        \hline
        F1    &0.995  &0.999 &0.973 &0.979 \\
        \hline
        FDR   &0.04\%  &0.00\% &0.25\% &0.26\% \\
        \hline
    \end{tabular}
    
    \label{tab:RLV_new}
\end{table}

%\vspace{-0.2in}
\begin{table}[h]
    \centering
    \caption{Spoof Detection Performance (Mirroring)}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
      {\bf Metrics}   & {\bf SVM\_BPA} & {\bf NN\_BPA} & {\bf SVM\_OSU} & {\bf NN\_OSU} \\
      \hline
        Accuracy &99.81\%  &99.93\% &98.53\% &98.92\% \\
        \hline
        Sensitivity    &98.36\%  &99.36\% &92.24\% &94.35\% \\
        \hline
        Precision   &99.94\%  &99.99\% &99.65\% &99.69\% \\
        \hline
        Specificity     &99.99\%  &100.00\% &99.93\% &99.94\% \\
        \hline
        F1    &0.991  &0.997 &0.958 &0.969 \\
        \hline
        FDR   &0.06\%  &0.01\% &0.35\% &0.31\% \\
        \hline
    \end{tabular}
    
    \label{tab:mirror_new}
\end{table}

%\vspace{-0.2in}
\begin{table}[h]
    \centering
    \caption{Spoof Detection Performance (Time Dilation)}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
      {\bf Metrics}   & {\bf SVM\_BPA} & {\bf NN\_BPA} & {\bf SVM\_OSU} & {\bf NN\_OSU} \\
      \hline
        Accuracy &99.39\%  &99.73\% &97.01\% &97.18\% \\
        \hline
        Sensitivity    &96.77\%  &98.71\% &85.00\% &85.54\% \\
        \hline
        Precision   &97.57\%  &98.84\% &98.30\% &98.78\% \\
        \hline
        Specificity     &99.71\%  &99.86\% &99.67\% &99.77\% \\
        \hline
        F1    &0.972  &0.988 &0.912 &0.917 \\
        \hline
        FDR   &2.43\%  &1.16\% &1.70\% &1.22\% \\
        \hline
    \end{tabular}
    \label{tab:dilation_new}
\end{table}

For all cases, we achieved high overall accuracy (ranging from 97.01\% to 99.97\%) and specificity (ranging from 99.67\% to 100.00\%), indicating that both techniques are effective in correctly identifying normal signals across the transmission level and distribution level. As for precision and FDR, in general both methods perform better on the BPA data. This is likely because the transmission level dataset has less noise compared to the distribution level dataset. 

For all cases, the sensitivity is relatively lower than other metrics, ranging from 85.00\% to 99.76\%. This metric measures the percentage of spoofed signals being correctly identified by the learning algorithms. This is attributed to the following two reasons. First, since there is only one PMU being spoofed, there are more normal examples than the spoofed ones (3.5-4 times in both datasets). Therefore the algorithms learn better in terms of identifying normal data. Second, the calculation of these metrics is based on individual examples/time points. Each cycle is an example. If a cycle is within the later 30 seconds of the spoofed minute, it is labeled as spoofed. However, the features representing this example are the correlations from a 300-cycle time window before this time point, which means that some of the spoofed examples have correlation features composed of mainly non-spoofed data. This fact may also affect the sensitivity. 

The overall performance of both techniques are high on both datasets, indicating that the features we use are generic across transmission level and distribution level.  


\subsection{ANN Training}

%It is worth noting that 
A key feature of neural networks is an iterative learning process in which examples are presented to the network one at a time, and the weights associated with the input values are adjusted each time.  Typically, this process is repeated for multiple iterations. In our experiments, we trained the network over 100 such iterations. However, there is a potential that the neural network achieves good performance with even less training time. To this end, we have measured the performance metrics after each time the network is trained, and the results are shown in Figure~\ref{fig:training}. For the larger BPA dataset, our neural network achieves near optimal performance after being trained 600 times (equivalent to approximately 6 minutes of CPU time on 1-core), while for the smaller OSU dataset, this number is decreased to approximately 150 (equivalent to less than 1 minute of CPU time on 1-core). This indicates that for a system with smaller numbers of PMUs, the neural network may achieve optimal performance with a much smaller number of epochs. \oldblue{Regardless, because the classifier is expected to only require retraining when the system configuration changes significantly, training can be viewed as an offline process.}

\begin{figure}[h]
    \centering
    \subfigure[BPA Data]{\includegraphics[width=0.4\textwidth]{figs/NN_BPA_Performance.png}}
    \subfigure[OSU Data]{\includegraphics[width=0.4\textwidth]{figs/NN_OSU_Performance.png}}
    \caption{ANN Performance vs. Training Times}
    \label{fig:training}
\end{figure}

\subsection{Spoof Detection Latency}

\oldblue{For each of our experiments, we have also measured the spoof detection latency, i.e., number of cycles after the spoof begins but before the classifier correctly identifies a string of 30 consecutive cycles as spoofed. This metric represents the promptness of our spoof detection method, which is critical in terms of applying this methodology in a real operational environment. }

\oldblue{Specifically, we calculated the minimum and maximum latency for detecting spoofs in one minute data, for each of the spoof procedures and datasets. We have also calculated the ``min of the max", which is the minimum of the max latency among all sites in each minute (the minimum latency of a spoof being detected by all sites). The latency results for SVM and NN are shown in Table~\ref{tab:svm_latency}, and  ~\ref{tab:nn_latency}, respectively. }




\oldblue{The experimental results show that the spoof detection methods works better on BPA data than on the OSU data in terms of latency. This is expected as the distribution-level OSU data are noisier than the transmission-level BPA data. Among the spoof procedures, Time Dilation is the most difficult to detect, indicated by longer latencies in all cases. The Time Dilation spoof uses real data to generate spoof signals, which are very similar to the real signals that a PMU would observe. }

\vspace{-0.22in}
\begin{table}[h]
    \centering
    \caption{Spoof Detection Latency (SVM)}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
      {\bf Metrics} & {\bf Min} & {\bf Max} & {\bf Min of Max} \\
      \hline
        OSU\_mirror &34  &135  &108  \\
        \hline
        OSU\_RLV &35  &294  &64  \\
        \hline
        OSU\_dilation &27  &443  &147  \\
        \hline
        BPA\_mirror &0  &80  &44  \\
        \hline
        BPA\_RLV &0  &118  &6  \\
        \hline
        BPA\_dilation &0  &174  &67  \\
        \hline
    \end{tabular}
    \label{tab:svm_latency}
\end{table}
\vspace{-0.25in}
\begin{table}[h]
    \centering
    \caption{Spoof Detection Latency (NN)}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
      {\bf Metrics} & {\bf Min} & {\bf Max} & {\bf Min of Max} \\
      \hline
        OSU\_mirror &10  &155  &115  \\
        \hline
        OSU\_RLV &12  &297  &99  \\
        \hline
        OSU\_dilation &31  &518  &157  \\
        \hline
        BPA\_mirror &7  &24  &19  \\
        \hline
        BPA\_RLV &2  &43  &24  \\
        \hline
        BPA\_dilation &11  &64  &35  \\
        \hline
    \end{tabular}
    \label{tab:nn_latency}
\end{table}


%\subsection{Computational Performance}

%\oldblue{System performance is dominated by two factors: feature extraction and training. While feature extraction needs to be performed both for training and on all PMU data to be classified by the learning system, training may only need to be performed periodically as system configuration changes.  To examine the scalability of the system,}



%\subsection{Improving Computational Performance}

%\oldblue{remove?/reduce? this section.}

%To further improve the performance of the neural network, we have carried out experiments to evaluate the training performance of a neural network on a distributed system using Tensorflow~\cite{abadi2016tensorflow}, an open-source software library for machine learning. We train our neural network using Tensorflow on three systems, with 1 node, 2 nodes, and 3 nodes. Each computing node has a 4-core Intel Xeon CPU @ 3.20GHz, and 8GB RAM. On each system, we vary the training time from 100 to 1000, and measure the computational performance, i.e., training time. The results are shown in Figure~\ref{fig:distributed}. 


%\begin{figure}[h]
%    \centering
%    \subfigure[BPA Data, Transmission Level]{\includegraphics[width=0.45\textwidth]{figs/one_two_three_BPA.png}}
%    \subfigure[OSU Data, Distribution Level]{\includegraphics[width=0.45\textwidth]{figs/one_two_three_OSU.png}}
%    \caption{ANN Training Performance on Distributed Systems}
%    \label{fig:distributed}
%\end{figure}

%On all three systems, the training performance is linearly related to the number of training examples. When running on a distributed system, the neural network on both datasets gain significant speedup, which indicates that the network can be easily scaled by leveraging distributed resources. This is essential when applying this approach to a much larger system, or when training the algorithm for online spoof detection, which has a higher requirement on the efficiency of the training. 

==> PMU data/6_discussion.tex <==
\section{Discussion}\label{sec:discussion}

==> PMU data/7_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

With information and communication technologies being integrated in modern power systems, big data and cyber security challenges become more pronounced. Historical cyber attack incidents indicate that spoofing is a common approach for disguising malicious activities. Spoofed data injected into a normal data stream make it difficult to identify the underlying attack. To address the challenges, we applied machine learning techniques to PMU data for the purpose of detecting spoofs. Specifically, we developed a generic set of correlation data based on features from PMU data. We then trained a SVM and an ANN. To perform a comprehensive evaluation, we used two datasets, one from BPA's transmission level 500 kV network, and the other from our inter-university, distribution level PMU network. Experimental results showed that both techniques perform well after being trained using the same set of features. In addition, the neural network approach demonstrates a good potential in achieving highly efficient training performance, via minimizing training iterations, or leveraging distributed resources. 

Work continues in multiple directions. First, we will explore classification accuracy and sensitivity (true positive rate) across a variety of spoofing circumstances. Additionally, we will explore specificity (true negative rate) across a large, contiguous sample. Second, we will investigate the possibilities of adjusting the performance of the spoof detection algorithm based on anticipated threat levels in response to cyber-defense intelligence. We expect to be able to modify detectability at the cost of increased computational complexity or increased false positive rate in response to anticipated events. Third, we will use principal component analysis to improve learning by reducing redundant information from the PMU data. 
